Exponential Mixing by Orthogonal Non-Monotonic Shears

Non-monotonic velocity profiles are an inherent feature of mixing flows obeying non-slip boundary conditions. There are, however, few known models of laminar mixing which incorporate this feature and have proven mixing properties. Here we present such a model, alternating between two non-monotonic shear flows which act in orthogonal (i.e. perpendicular) directions. Each shear is defined by an independent variable, giving a two-dimensional parameter space within which we prove the mixing property over open subsets. Within these mixing windows, we use results from the billiards literature to establish exponential mixing rates. Outside of these windows, we find large parameter regions where elliptic islands persist, leading to poor mixing. Finally, we comment on the challenges of extending these mixing windows and the potential for a non-exponential mixing rate at particular parameter values.

==> sections/newGraph.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[scale=2.3]
    % NOTE: to change scale of whole figure you must also change the global scale below
    \node at (2.495,2.54) {
    
    \definecolor{white}{RGB}{255,255,255}

% Exported .svg from Desmos, converted to tikz via svg2tikz python package
\def \globalscale {0.231*23/25}
\begin{tikzpicture}[y=0.80pt, x=0.80pt, yscale=-\globalscale, xscale=\globalscale, inner sep=0pt, outer sep=0pt]
\begin{scope}[scale=2.000]
    \path[fill=white,rounded corners=0.0000cm] (0.0000,0.0000) rectangle (1000.0000,1000.0000);



        \path[draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (9.3039,989.6961) -- (9.3039,989.6961) -- (9.3039,9.3039);



        \path[draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (9.3039,9.3039) -- (9.3039,9.3039) -- (989.6961,9.3039);



        \path[draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (9.3039,989.6961) -- (9.3039,989.6961) -- (989.6961,989.6961);



        \path[draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (989.6961,989.6961) -- (989.6961,989.6961) -- (989.6961,9.3039);


        % HYPERBOLICITY
        \path[fill=gray!10,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (9.3039,989.6961) -- (9.3039,744.5980) -- (9.3039,744.5980) -- (45.3984,735.2295) -- (79.8223,725.6021) -- (112.5371,715.7524) -- (143.5430,705.7141) -- (173.3281,695.3531) -- (201.6484,684.7752) -- (228.7480,673.9160) -- (254.6270,662.7987) -- (279.5293,651.3358) -- (303.4551,639.5389) -- (326.6484,627.2905) -- (348.8652,614.7263) -- (370.3496,601.7191) -- (391.1016,588.2688) -- (411.3652,574.2035) -- (430.8965,559.6811) -- (449.6953,544.7112) -- (467.5176,529.5236) -- (484.3633,514.1833) -- (500.2324,498.7665) -- (515.3691,483.0999) -- (529.7734,467.2339) -- (543.6895,450.9323) -- (557.1172,434.2085) -- (570.0566,417.0802) -- (582.5078,399.5705) -- (594.4707,381.7083) -- (605.9453,363.5287) -- (617.1758,344.6515) -- (627.9180,325.4984) -- (638.4160,305.6487) -- (648.6699,285.0809) -- (658.6797,263.7737) -- (668.4453,241.7066) -- (677.9668,218.8599) -- (687.2441,195.2155) -- (696.2773,170.7566) -- (705.0664,145.4686) -- (713.6113,119.3394) -- (722.1562,91.5412) -- (730.4570,62.7825) -- (738.5137,33.0519) -- (744.5980,9.3039) -- (989.6961,9.3039);

        \path[fill=gray!10,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (9.3039,989.6961) -- (254.4020,989.6961) -- (254.4020,989.6961) -- (262.4615,958.4844) -- (270.7092,928.5365) -- (279.1173,899.8906) -- (287.7688,872.2214) -- (296.5457,845.8542) -- (305.5369,820.4635) -- (314.7295,796.0495) -- (324.1076,772.6120) -- (333.7944,749.8255) -- (343.6413,728.0156) -- (353.7828,706.8568) -- (364.2171,686.3490) -- (374.9407,666.4922) -- (385.9478,647.2865) -- (397.2300,628.7318) -- (408.7761,610.8281) -- (420.8012,593.2500) -- (433.3289,575.9974) -- (446.1258,559.3958) -- (459.4445,543.1198) -- (473.3091,527.1693) -- (487.7446,511.5443) -- (502.7770,496.2448) -- (518.7846,480.9453) -- (535.4903,465.9714) -- (552.9281,451.3229) -- (571.5612,436.6745) -- (591.0581,422.3516) -- (611.4642,408.3542) -- (632.3005,395.0078) -- (654.0668,381.9870) -- (676.2019,369.6172) -- (699.2654,357.5729) -- (723.2900,345.8542) -- (748.3075,334.4609) -- (774.3481,323.3932) -- (801.4400,312.6510) -- (829.6085,302.2344) -- (858.8754,292.1432) -- (890.3078,282.0521) -- (923.0231,272.2865) -- (957.0435,262.8464) -- (989.6961,254.4020) -- (989.6961,9.3039);


        % MIXING WINDOWS
        \path[fill=gray!40,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (221.8336,989.4902) -- (221.8336,989.4902) -- (230.6817,908.9433) -- (235.8281,857.9290) -- (239.5646,815.9062) -- (241.9118,784.1282) -- (243.4491,756.5801) --     (242.4199,755.5509) -- (242.4199,755.5509) -- (214.8717,757.0882) -- (183.0938,759.4355) -- (141.0710,763.1719) -- (90.0567,768.3183) -- (9.5098,777.1664) -- (9.5098,989.4902);

        \path[fill=gray!40,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (777.1664,9.5098) -- (777.1664,9.5098) -- (769.6814,77.6250) -- (764.2275,131.4150) -- (760.6707,170.5180) -- (757.4084,212.4865) -- (755.5602,242.4199) -- (756.5801,243.4491) -- (756.5801,243.4491) -- (784.1283,241.9118) -- (803.0731,240.5731) -- (803.0731,240.5731) -- (835.5474,237.8911) -- (886.2188,233.0369) -- (956.5313,225.5233) -- (989.4902,221.8336) -- (989.6961,9.3039);


        % EXPONENTIAL MIXING WINDOWS
        \path[fill=gray!80,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00](9.5098,989.4902) -- (221.8336,989.4902) -- (221.8336,989.4902) -- (230.6817,908.9433) -- (235.8281,857.9290) -- (238.0254,831.8217) -- (238.0254,831.8217) -- (235.4516,824.6953) -- (232.8931,818.8413) -- (231.4307,815.9062) -- (225.6891,806.4422) -- (223.8117,803.8898) -- (216.4890,795.6946) -- (211.6582,791.4400) -- (209.2911,789.5762) -- (209.2911,789.5762) -- (205.0664,784.4073) -- (200.6719,779.9106) -- (191.3599,772.4838) -- (190.5775,771.9609) -- (179.0758,765.5994) -- (170.8489,762.2332) -- (167.1783,760.9746) -- (141.0710,763.1719) -- (90.0567,768.3183) -- (9.5098,777.1664) -- (9.5098,989.4902);

        \path[fill=gray!80,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00](989.6961,9.3039) -- (777.1664,9.5098) -- (777.1664,9.5098) -- (769.6814,77.6250) -- (764.2275,131.4150) -- (760.9746,167.1783) -- (760.9746,167.1783) -- (761.1063,167.5812) -- (761.1063,167.5812) -- (763.5484,174.3047) -- (766.1069,180.1587) -- (767.5693,183.0937) -- (773.3109,192.5578) -- (775.1883,195.1102) -- (782.5110,203.3054) -- (787.3418,207.5600) -- (789.4949,209.2305) -- (789.7089,209.4238) -- (789.7089,209.4238) -- (790.3502,210.2721) -- (790.3502,210.2721) -- (795.2782,216.0527) -- (798.3281,219.0894) -- (807.6401,226.5162) -- (808.4225,227.0391) -- (819.9242,233.4006) -- (828.1511,236.7668) -- (831.8217,238.0254) -- (835.5474,237.8911) -- (886.2188,233.0369) -- (956.5313,225.5233) -- (989.4902,221.8336) -- (989.6961,9.3039);

        % PERIOD 2
        \path[pattern= dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (499.5000,989.6961) -- (499.5000,499.5000) -- (989.6961 ,499.5000) -- (989.6961 ,989.6961) -- (499.5000,989.6961);

        \path[pattern= dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00]  (499.5000,499.5000) -- (499.5000, 9.3039) -- (9.3039 ,9.3039) -- (9.3039, 499.5000) -- (499.5000,499.5000);


        \path[pattern= dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (126.9711,618.3268) -- (126.9711,618.3268) -- (51.2362,600.4115) -- (9.3039,590.7454) -- (9.3039,662.8987) -- (9.3039,662.8987) -- (41.2480,651.8920) -- (72.0098,640.5685) -- (101.5508,628.9560) -- (126.9711,618.3268);



        \path[pattern = dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (380.6732,872.0289) -- (380.6732,872.0289) -- (396.2285,937.6325) -- (408.2546,989.6961) -- (336.1013,989.6961) -- (336.1013,989.6961) -- (345.6937,961.7396) -- (355.3931,935.0469) -- (365.2818,909.3307) -- (375.4795,884.2656) -- (380.6732,872.0289);



        \path[pattern = dots,draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (989.6961,408.2546) -- (989.6961,408.2546) -- (903.3901,388.1719) -- (872.0289,380.6732) -- (872.0289,380.6732) -- (872.0289,380.6732) -- (900.1348,368.9565) -- (929.4316,357.5051) -- (959.9492,346.3272) -- (989.6961,336.1013);



        \path[pattern = dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (590.7454,9.3039) -- (590.7454,9.3039) -- (608.1426,84.2567) -- (618.3268,126.9711) -- (618.3268,126.9711) -- (618.3268,126.9711) -- (628.4927,102.6901) -- (638.5444,77.2995) -- (648.2889,51.2578) -- (657.8431,24.2396) -- (662.8987,9.3039);



        \path[pattern=dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (224.2290,499.5000) -- (224.2290,499.5000) -- (231.6777,535.7173) -- (237.1550,563.9524) -- (237.1550,563.9524) -- (237.1550,563.9524) -- (260.7305,550.1834) -- (283.4355,536.0539) -- (305.6523,521.3202) -- (327.1367,506.1325) -- (336.1013,499.5000);



        \path[pattern=dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (499.5000,774.7710) -- (499.5000,774.7710) -- (457.1118,766.1016) -- (435.0476,761.8450) --  (435.0476,761.8450) -- (435.0476,761.8450) -- (446.7654,741.6875) -- (458.9566,721.8307) -- (471.4125,702.6250) -- (484.3487,683.7448) -- (497.7874,665.1901) -- (499.5000,662.8987);



        \path[pattern = dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (761.8450,435.0476) -- (761.8450,435.0476) -- (769.2754,473.0152) -- (774.7710,499.5000) -- (662.8987,499.5000) -- (662.8987,499.5000) -- (684.3145,483.9478) -- (706.2871,468.9844) -- (728.7480,454.6333) -- (751.9414,440.7252) -- (761.8450,435.0476);



        \path[pattern = dots, draw=black,draw opacity=0.900,line cap=round,line join=round,line width=0.500pt,miter limit=10.00] (563.9524,237.1550) -- (563.9524,237.1550) -- (520.7843,228.6667) -- (499.5000,224.2290) -- (499.5000,336.1013) -- (499.5000,336.1013) -- (512.8100,317.8594) -- (525.8453,298.9792) -- (538.3940,279.7734) -- (550.6736,259.9167) -- (562.6735,239.4089) -- (563.9524,237.1550);




\end{scope}

\end{tikzpicture}
   };

 \draw[->] (0,0) -- (0,2.3);
 \draw[->] (0,0) -- (2.3,0);
 
 \node at (5.1,-0.1) {1};
 \node at (-0.075,5.1) {1};
 \node at (-0.075,-0.075) {0};
 
\node at (2.3,-0.1) {$\xi$};
 \node at (-0.075,2.3) {$\eta$};
 

\filldraw[pattern = dots] (5.5,3.3) rectangle (5.7,3.5);
\node at (6.28,3.38) {Elliptic islands};

\filldraw[fill=gray!80] (5.5,2.7) rectangle (5.7,2.9);
\node at (6.2,2.78) {Exp. mixing};

\node at (5.6,2.5) {$\subset$};

\filldraw[fill = gray!40] (5.5,2.1) rectangle (5.7,2.3);
\node at (6.02,2.18) {Mixing};

\node at (5.6,1.9) {$\subset$};

\filldraw[fill = gray!10] (5.5,1.5) rectangle (5.7,1.7);
\node at (6.15,1.58) {Hyperbolic};

    \end{tikzpicture}
    \caption{dsfsd}
    \label{fig:fullParameterSpace}
\end{figure}
